Monte Carlo Rendering to Diffusion Curves with Differential BEM

We present a method for generating vector graphics, in the form of diffusion curves, directly from noisy samples produced by a Monte Carlo renderer. While generating raster images from 3D geometry via Monte Carlo raytracing is commonplace, there is no corresponding practical approach for robustly and directly extracting editable vector images with shading information from 3D geometry. To fill this gap, we formulate the problem as a stochastic optimization problem over the space of geometries and colors of diffusion curve handles, and solve it with the Levenberg-Marquardt algorithm. At the core of our method is a novel differential boundary element method (BEM) framework that reconstructs colors from diffusion curve handles and computes gradients with respect to their parameters, requiring the expensive matrix factorization only once at the beginning of the optimization. Unlike triangulation-based techniques that require a clean domain decomposition, our method is robust to geometrically challenging scenarios, such as intersecting diffusion curves, and to color noise in the target image, enabling the direct use of noisy Monte Carlo samples without requiring a converged, error-free input image. We demonstrate the robustness and broad applicability of our approach across several test cases. Finally, we highlight several open questions raised by our work, which spans both theory and applications.

==> Figures/results/cb2_data/adamw_1e_1_step_vs_rmse_tonemapped_abs.tex <==
0 0.1606356
1 0.05598996
2 0.35984352
3 0.22168855
4 0.39445028
5 0.20930706
6 0.14175296
7 0.19397259
8 0.28964424
9 0.17208026
10 0.14030974
11 0.1751683
12 0.12962139
13 0.1292357
14 0.15101774
15 0.12019386
16 0.09260716
17 0.099769905
18 0.09495282
19 0.08576575
20 0.0877495
21 0.08000499
22 0.06657807
23 0.0757849
24 0.0680223
25 0.058914833
26 0.060451403
27 0.06131918
28 0.05433721
29 0.053503655
30 0.051609937
31 0.052286383
32 0.047048718
33 0.04821574
34 0.045364205
35 0.04965883
36 0.04562222
37 0.04308985
38 0.03960467
39 0.039511956
40 0.038715057
41 0.035192646
42 0.03515836
43 0.034185734
44 0.033885997
45 0.03279504
46 0.03216284
47 0.034913935
48 0.03791853
49 0.044233914
50 0.04125326
51 0.030604599
52 0.035647232
53 0.02914657
54 0.032653645
55 0.028460672
56 0.02991273
57 0.02823883
58 0.02767979
59 0.02810889
60 0.033470042
61 0.031996287
62 0.027459374
63 0.028033897
64 0.028682709
65 0.025718622
66 0.027521454
67 0.026565857
68 0.024558526
69 0.026686514
70 0.024335692
71 0.024814233
72 0.024478791
73 0.02391692
74 0.023897145
75 0.023219086
76 0.023554461
77 0.022931635
78 0.023447547
79 0.022797566
80 0.022486484
81 0.022270544
82 0.022498127
83 0.022665681
84 0.023401372
85 0.022099378
86 0.021989992
87 0.02168514
88 0.021578353
89 0.021088434
90 0.021028444
91 0.02226876
92 0.021476798
93 0.021163726
94 0.02118734
95 0.020731548
96 0.021019584
97 0.021304859
98 0.021634758
99 0.021422433
100 0.022879804


==> Figures/results/cb2_data/adamw_1e_2_step_vs_rmse_tonemapped_abs.tex <==
0 0.1606356
1 0.055989902
2 0.052177716
3 0.04621128
4 0.041060757
5 0.036242265
6 0.032521695
7 0.029765366
8 0.02813153
9 0.02640604
10 0.024999736
11 0.023900088
12 0.023853702
13 0.022879582
14 0.021815324
15 0.02119145
16 0.020793905
17 0.020854818
18 0.02015334
19 0.020222306
20 0.019770466
21 0.019887552
22 0.02017119
23 0.019089812
24 0.019267367
25 0.018666206
26 0.018898763
27 0.019410968
28 0.018748717
29 0.020109946
30 0.019656666
31 0.01906768
32 0.01990676
33 0.018906234
34 0.020053023
35 0.02024327
36 0.018823713
37 0.018810073
38 0.018450858
39 0.018583247
40 0.0198015
41 0.018326305
42 0.01813237
43 0.018195515
44 0.017724296
45 0.017546741
46 0.01823859
47 0.017774353
48 0.017120704
49 0.017417395
50 0.017197285
51 0.0180257
52 0.018982766
53 0.017623784
54 0.0169404
55 0.01698493
56 0.016575051
57 0.016452534
58 0.016796963
59 0.017444463
60 0.017329128
61 0.016978057
62 0.017308392
63 0.017029516
64 0.016628087
65 0.016706364
66 0.016804362
67 0.016392415
68 0.016217886
69 0.016215183
70 0.016056199
71 0.016150054
72 0.016114974
73 0.01594305
74 0.015870195
75 0.015865114
76 0.015652055
77 0.015688438
78 0.018281363
79 0.017101828
80 0.017318217
81 0.016679723
82 0.016980674
83 0.016521202
84 0.016777096
85 0.016384521
86 0.015987325
87 0.016404467
88 0.015757335
89 0.016351633
90 0.01637815
91 0.015863452
92 0.015493858
93 0.01592585
94 0.015483231
95 0.015590379
96 0.015548521
97 0.015524425
98 0.015564468
99 0.015513837
100 0.015357238


==> Figures/results/cb2_data/adamw_1e_3_step_vs_rmse_tonemapped_abs.tex <==
0 0.1606356
1 0.055989634
2 0.05511482
3 0.05431733
4 0.05358379
5 0.052865192
6 0.052154686
7 0.05144364
8 0.0507364
9 0.050011806
10 0.04928961
11 0.04855199
12 0.04781677
13 0.047096677
14 0.046370063
15 0.045658186
16 0.044946816
17 0.04424012
18 0.043536164
19 0.04284031
20 0.042145103
21 0.04146244
22 0.040785406
23 0.040125057
24 0.039465405
25 0.038825244
26 0.03818788
27 0.03757148
28 0.03697612
29 0.036391642
30 0.035822175
31 0.035266716
32 0.034716677
33 0.034173694
34 0.03368461
35 0.033208206
36 0.032734443
37 0.032265067
38 0.031784322
39 0.031309146
40 0.030827316
41 0.0303779
42 0.029926939
43 0.029494947
44 0.029073736
45 0.028673716
46 0.02829853
47 0.027944356
48 0.027601752
49 0.027276874
50 0.026967755
51 0.026729096
52 0.026511902
53 0.026276726
54 0.026033606
55 0.02575368
56 0.025509054
57 0.025221266
58 0.02497872
59 0.024716234
60 0.024512168
61 0.024299419
62 0.024113992
63 0.023922548
64 0.023755113
65 0.02357991
66 0.02344061
67 0.023311691
68 0.023203246
69 0.023100536
70 0.022993065
71 0.022924988
72 0.022794008
73 0.022654908
74 0.022500372
75 0.022334801
76 0.022190548
77 0.022071715
78 0.021945912
79 0.021864356
80 0.021804316
81 0.02172622
82 0.021625577
83 0.021549681
84 0.02150124
85 0.02142071
86 0.021335345
87 0.021203991
88 0.021109156
89 0.02097818
90 0.020873228
91 0.020782059
92 0.020661103
93 0.020579888
94 0.020507777
95 0.020444602
96 0.020385675
97 0.020336611
98 0.020282345
99 0.02022541
100 0.020126488


==> Figures/results/cb2_data/baseline_step_vs_num_handles.tex <==
0 500
1 500
2 500
3 500
4 499
5 499
6 499
7 499
8 499
9 499
10 499
11 499
12 499
13 499
14 499
15 499
16 499
17 499
18 499
19 499
20 499
21 499
22 499
23 499
24 499
25 499
26 499
27 499
28 499
29 499
30 499
31 499
32 499
33 499
34 499
35 499
36 499
37 499
38 499
39 499
40 499
41 499
42 499
43 499
44 499
45 499
46 499
47 499
48 499
49 499
50 499
51 499
52 499
53 499
54 499
55 499
56 499
57 499
58 499
59 499
60 499
61 499
62 499
63 499
64 499
65 499
66 499
67 499
68 499
69 499
70 499
71 499
72 499
73 499
74 499
75 499
76 499
77 499
78 499
79 499
80 499
81 499
82 499
83 499
84 499
85 499
86 499
87 499
88 499
89 499
90 499
91 499
92 499
93 499
94 499
95 499
96 499
97 499
98 499
99 499
100 499


==> Figures/results/cb2_data/baseline_step_vs_rmse_tonemapped_abs.tex <==
0 0.1606356
1 0.055989023
2 0.032755196
3 0.023373434
4 0.02057802
5 0.018183284
6 0.018122522
7 0.017350027
8 0.016838465
9 0.01620746
10 0.016295448
11 0.015601329
12 0.015656065
13 0.015460631
14 0.015489816
15 0.015008759
16 0.015047533
17 0.015112644
18 0.01491382
19 0.014956692
20 0.01457793
21 0.014664542
22 0.01455961
23 0.014490882
24 0.014414612
25 0.01582013
26 0.015903598
27 0.016232824
28 0.014980908
29 0.015649684
30 0.014905119
31 0.014559368
32 0.014537218
33 0.015223005
34 0.016431134
35 0.016768018
36 0.015509329
37 0.015140443
38 0.0149948
39 0.0147772115
40 0.014724289
41 0.014480225
42 0.014324393
43 0.014329677
44 0.014349459
45 0.014331783
46 0.014584872
47 0.014473597
48 0.015109147
49 0.015068574
50 0.014936699
51 0.014762978
52 0.014944284
53 0.014774828
54 0.014995647
55 0.014776368
56 0.014745194
57 0.01478513
58 0.014593186
59 0.014494804
60 0.015093111
61 0.014728631
62 0.015410347
63 0.01434578
64 0.013852726
65 0.014257928
66 0.014180157
67 0.014127254
68 0.014004198
69 0.01384862
70 0.014158409
71 0.014119541
72 0.014073512
73 0.013972953
74 0.013708089
75 0.013666984
76 0.014435182
77 0.014305828
78 0.014456843
79 0.014672652
80 0.014211912
81 0.014275172
82 0.014286513
83 0.01429626
84 0.014309049
85 0.014371242
86 0.01424791
87 0.013949863
88 0.013732531
89 0.014111664
90 0.014021333
91 0.014002965
92 0.013880655
93 0.013881341
94 0.013853312
95 0.013645335
96 0.013854296
97 0.013800655
98 0.013906911
99 0.013956801
100 0.013788123


==> Figures/results/cb2_data/nopruning_step_vs_rmse_tonemapped_abs.tex <==
0 0.1606356
1 0.055989753
2 0.032925166
3 0.022761468
4 0.02069395
5 0.017637566
6 0.016820878
7 0.01646106
8 0.01649938
9 0.01605504
10 0.01578774
11 0.015467206
12 0.015529972
13 0.015592801
14 0.015028953
15 0.014943012
16 0.0149689885
17 0.014736598
18 0.0147213265
19 0.014721984
20 0.014756013
21 0.014925813
22 0.014393278
23 0.016239826
24 0.015410209
25 0.015389778
26 0.014872986
27 0.0150349885
28 0.014703882
29 0.014818185
30 0.014101924
31 0.015162059
32 0.014323852
33 0.014512074
34 0.015086099
35 0.01383121
36 0.014295564
37 0.014139047
38 0.013844814
39 0.013981533
40 0.013858158
41 0.013751834
42 0.013584365
43 0.013671453
44 0.013828684
45 0.013786168
46 0.01416758
47 0.013912072
48 0.015021021
49 0.015047851
50 0.0139857195
51 0.014088652
52 0.013960239
53 0.014192495
54 0.014013937
55 0.014282903
56 0.014221926
57 0.014109419
58 0.01398083
59 0.014842687
60 0.014282213
61 0.014068431
62 0.013835999
63 0.013796441
64 0.013923296
65 0.01378359
66 0.014061816
67 0.013805695
68 0.013846284
69 0.013891379
70 0.013964085
71 0.013966988
72 0.013797394
73 0.013770778
74 0.013608034
75 0.013805113
76 0.0138064185
77 0.013768102
78 0.013828556
79 0.013806435
80 0.014038615
81 0.015249501
82 0.014707457
83 0.014975642
84 0.01431264
85 0.0138676185
86 0.014119656
87 0.014287179
88 0.014154095
89 0.0138815
90 0.014237812
91 0.014195452
92 0.014346378
93 0.014217252
94 0.0137907285
95 0.014141031
96 0.013946743
97 0.014103441
98 0.014016734
99 0.013793317
100 0.014763551


==> Figures/results/cb2_data/smallersmoothing_step_vs_rmse_tonemapped_abs.tex <==
0 0.1606356
1 0.05599018
2 0.03360676
3 0.026172152
4 0.024419487
5 0.022898467
6 0.022857696
7 0.022474444
8 0.022284025
9 0.022161938
10 0.021856416
11 0.021654343
12 0.021377757
13 0.02133223
14 0.021395708
15 0.020992206
16 0.020662313
17 0.02015331
18 0.020027205
19 0.019838747
20 0.019982561
21 0.019523945
22 0.019381762
23 0.019796578
24 0.019744264
25 0.019085176
26 0.019073227
27 0.01905322
28 0.019204754
29 0.018887961
30 0.019004377
31 0.018801667
32 0.018905893
33 0.01882689
34 0.02139095
35 0.018705882
36 0.018670944
37 0.018579083
38 0.017692791
39 0.017596418
40 0.017201276
41 0.017513568
42 0.017310146
43 0.017292753
44 0.017065266
45 0.017033767
46 0.017407058
47 0.01700778
48 0.016624864
49 0.0173044
50 0.01664932
51 0.016967092
52 0.017033387
53 0.016409814
54 0.016374702
55 0.016419819
56 0.016318496
57 0.016320296
58 0.01640247
59 0.016483532
60 0.017201794
61 0.017112665
62 0.016968504
63 0.016881108
64 0.016759729
65 0.016565533
66 0.01628599
67 0.016278466
68 0.01623607
69 0.016171599
70 0.016157977
71 0.016134217
72 0.016149303
73 0.016252961
74 0.016321728
75 0.016257372
76 0.016217533
77 0.016263813
78 0.016022248
79 0.016189761
80 0.01667246
81 0.016898984
82 0.016454522
83 0.016439864
84 0.016415536
85 0.01665549
86 0.016255086
87 0.016131096
88 0.016319666
89 0.016392114
90 0.016346764
91 0.016253907
92 0.016382752
93 0.01652477
94 0.016345508
95 0.016363975
96 0.01619319
97 0.016332963
98 0.01619337
99 0.016098501
100 0.01614693


==> Figures/results/cb2_data/sparsity_100x_step_vs_num_handles.tex <==
0 500
1 500
2 500
3 301
4 299
5 294
6 294
7 289
8 287
9 253
10 220
11 213
12 212
13 208
14 206
15 199
16 186
17 180
18 176
19 173
20 170
21 164
22 152
23 150
24 150
25 150
26 150
27 150
28 149
29 149
30 147
31 147
32 147
33 147
34 147
35 146
36 146
37 146
38 146
39 146
40 145
41 144
42 144
43 144
44 144
45 144
46 144
47 144
48 144
49 144
50 144
51 144
52 144
53 144
54 144
55 144
56 144
57 144
58 144
59 144
60 144
61 144
62 144
63 144
64 144
65 144
66 144
67 144
68 144
69 144
70 144
71 144
72 144
73 144
74 144
75 144
76 144
77 144
78 144
79 144
80 144
81 144
82 144
83 144
84 144
85 144
86 144
87 144
88 144
89 144
90 144
91 144
92 144
93 144
94 144
95 144
96 144
97 144
98 144
99 144
100 144


==> Figures/results/cb2_data/sparsity_100x_step_vs_rmse_tonemapped_abs.tex <==
0 0.1606356
1 0.055990595
2 0.055740036
3 0.055561475
4 0.05552555
5 0.05549239
6 0.055379648
7 0.055010412
8 0.054515366
9 0.05430464
10 0.053329397
11 0.05076772
12 0.048707493
13 0.048215106
14 0.046281587
15 0.045631662
16 0.04318642
17 0.039918717
18 0.037480827
19 0.03466238
20 0.03400926
21 0.03315094
22 0.032167844
23 0.03144452
24 0.030847248
25 0.029993374
26 0.029871605
27 0.029253263
28 0.02847938
29 0.028432721
30 0.027704261
31 0.027718151
32 0.027409006
33 0.026923768
34 0.02702819
35 0.02670849
36 0.026678728
37 0.026591955
38 0.026518889
39 0.026215758
40 0.026211103
41 0.02588088
42 0.025650255
43 0.025402745
44 0.024998108
45 0.02473957
46 0.02456591
47 0.024439916
48 0.024343014
49 0.024274707
50 0.024040451
51 0.023956379
52 0.023999242
53 0.023926651
54 0.023817789
55 0.023741996
56 0.023558429
57 0.023472726
58 0.023416623
59 0.023376822
60 0.023561064
61 0.023180883
62 0.023104357
63 0.022856437
64 0.022823125
65 0.022784913
66 0.02270391
67 0.022629812
68 0.02266695
69 0.022648169
70 0.02266635
71 0.022663634
72 0.02272348
73 0.022595834
74 0.022643963
75 0.022613965
76 0.022641735
77 0.022626596
78 0.022559753
79 0.02267473
80 0.0227536
81 0.022549802
82 0.022541387
83 0.022738192
84 0.022454798
85 0.022502825
86 0.022418262
87 0.022474544
88 0.022541411
89 0.022528825
90 0.022473825
91 0.022450497
92 0.02245824
93 0.02240021
94 0.02239527
95 0.022471847
96 0.022457056
97 0.022393608
98 0.022380179
99 0.022377532
100 0.022181658


==> Figures/results/cb2_data/sparsity_10x_step_vs_num_handles.tex <==
0 500
1 500
2 500
3 481
4 479
5 475
6 468
7 466
8 464
9 462
10 457
11 452
12 446
13 442
14 442
15 440
16 436
17 435
18 434
19 431
20 431
21 431
22 426
23 425
24 418
25 417
26 417
27 416
28 416
29 416
30 414
31 413
32 413
33 412
34 412
35 412
36 412
37 410
38 408
39 405
40 405
41 405
42 405
43 405
44 405
45 405
46 405
47 405
48 405
49 405
50 405
51 405
52 404
53 404
54 404
55 404
56 404
57 404
58 404
59 404
60 404
61 404
62 404
63 401
64 401
65 401
66 401
67 401
68 401
69 401
70 401
71 401
72 401
73 401
74 401
75 401
76 401
77 401
78 401
79 401
80 401
81 401
82 401
83 401
84 400
85 400
86 400
87 400
88 400
89 400
90 400
91 400
92 400
93 400
94 399
95 399
96 399
97 399
98 399
99 399
100 399


==> Figures/results/cb2_data/sparsity_10x_step_vs_rmse_tonemapped_abs.tex <==
0 0.1606356
1 0.05598984
2 0.054531503
3 0.053912807
4 0.053779975
5 0.05345632
6 0.05273982
7 0.050955128
8 0.0474489
9 0.04149236
10 0.037023377
11 0.03541711
12 0.031450838
13 0.030881593
14 0.028158821
15 0.027351206
16 0.026641952
17 0.025532698
18 0.024619555
19 0.024220608
20 0.02326667
21 0.022893045
22 0.022503313
23 0.022384288
24 0.022212
25 0.02225857
26 0.022069087
27 0.021986183
28 0.022331325
29 0.021941999
30 0.021800412
31 0.021688063
32 0.021491854
33 0.02150411
34 0.021378879
35 0.021567475
36 0.021355528
37 0.02126848
38 0.02133455
39 0.02101108
40 0.020953063
41 0.020849695
42 0.020780565
43 0.020674404
44 0.020600196
45 0.020540247
46 0.020627474
47 0.020316219
48 0.020486021
49 0.020227348
50 0.01998056
51 0.019524882
52 0.019272925
53 0.019274589
54 0.019108512
55 0.019133892
56 0.019031502
57 0.018818544
58 0.018706584
59 0.019166844
60 0.018873744
61 0.018746193
62 0.01873514
63 0.018608946
64 0.018544152
65 0.018550936
66 0.018542992
67 0.018604401
68 0.018530732
69 0.018538326
70 0.018481595
71 0.0184856
72 0.018475832
73 0.018500783
74 0.018521586
75 0.01849091
76 0.01849147
77 0.018482378
78 0.01845244
79 0.018461555
80 0.018678382
81 0.018963067
82 0.018475054
83 0.018453175
84 0.018530391
85 0.018533751
86 0.018457314
87 0.018457312
88 0.01854189
89 0.018491622
90 0.018509075
91 0.018361408
92 0.018409913
93 0.018432897
94 0.01838347
95 0.018286245
96 0.01835417
97 0.018358411
98 0.01829814
99 0.018324737
100 0.018360997


==> Figures/results/cb2_data/sparsity_1x_step_vs_num_handles.tex <==
0 500
1 500
2 500
3 499
4 498
5 498
6 498
7 498
8 498
9 495
10 494
11 494
12 494
13 492
14 492
15 491
16 491
17 491
18 491
19 490
20 490
21 490
22 490
23 490
24 490
25 490
26 490
27 488
28 487
29 487
30 487
31 486
32 486
33 486
34 486
35 486
36 486
37 486
38 486
39 486
40 486
41 485
42 485
43 485
44 485
45 485
46 485
47 485
48 484
49 484
50 483
51 482
52 482
53 482
54 482
55 481
56 481
57 481
58 480
59 480
60 479
61 479
62 479
63 479
64 478
65 478
66 478
67 478
68 476
69 475
70 475
71 475
72 474
73 474
74 474
75 474
76 474
77 474
78 473
79 472
80 471
81 471
82 471
83 470
84 470
85 470
86 470
87 470
88 470
89 470
90 470
91 470
92 470
93 469
94 469
95 468
96 468
97 468
98 468
99 467
100 464


==> Figures/results/cb2_data/sparsity_1x_step_vs_rmse_tonemapped_abs.tex <==
0 0.1606356
1 0.055990703
2 0.04960912
3 0.04693965
4 0.044804953
5 0.04167285
6 0.035961844
7 0.032512505
8 0.029845696
9 0.026751796
10 0.0252622
11 0.023951132
12 0.02302781
13 0.0220799
14 0.021698844
15 0.02126885
16 0.021084907
17 0.020893835
18 0.020768173
19 0.020485314
20 0.020118069
21 0.020077761
22 0.020320749
23 0.019995179
24 0.019438062
25 0.019197965
26 0.019176088
27 0.019111158
28 0.019022513
29 0.01912501
30 0.018760508
31 0.018604795
32 0.01867262
33 0.0185963
34 0.01895238
35 0.018848304
36 0.018653827
37 0.018551074
38 0.018497957
39 0.018935971
40 0.018385632
41 0.018292839
42 0.018147344
43 0.018072488
44 0.018091565
45 0.01899016
46 0.018132936
47 0.017847355
48 0.019095283
49 0.018289652
50 0.017859058
51 0.017772317
52 0.017422017
53 0.017094791
54 0.016942235
55 0.016722482
56 0.016580438
57 0.016522476
58 0.017368756
59 0.038316928
60 0.03676134
61 0.033680942
62 0.028920755
63 0.0228399
64 0.018674098
65 0.017892912
66 0.016828379
67 0.01642025
68 0.016367594
69 0.016153047
70 0.016190587
71 0.016106617
72 0.016568499
73 0.016449377
74 0.01632906
75 0.016261216
76 0.016779628
77 0.016567275
78 0.016351346
79 0.017428067
80 0.016657008
81 0.01629598
82 0.01619951
83 0.016565932
84 0.01651677
85 0.016217005
86 0.01595701
87 0.01587162
88 0.015826998
89 0.015800744
90 0.015831115
91 0.015876457
92 0.015871514
93 0.017350407
94 0.016592132
95 0.016083367
96 0.016053522
97 0.016201343
98 0.016052496
99 0.015927298
100 0.016336506


==> Figures/results/cb4_step_vs_rmse_tonemapped_abs.tex <==
0 0.16297957
1 0.063312106
2 0.03834829
3 0.03403874
4 0.03211042
5 0.029224684
6 0.02629089
7 0.022837136
8 0.024767717
9 0.023874521
10 0.02162288
11 0.019965831
12 0.021557903
13 0.01860245
14 0.018114593
15 0.019649336
16 0.019562647
17 0.017637033
18 0.016397938
19 0.016863324
20 0.016155213
21 0.015805382
22 0.0152568
23 0.015286936
24 0.015028946
25 0.014925246
26 0.0151008265
27 0.015177418
28 0.016192216
29 0.015848018
30 0.01545845
31 0.015536212
32 0.0155048575
33 0.015514796
34 0.015449454
35 0.015603606
36 0.015423731
37 0.015673432
38 0.015048305
39 0.015013024
40 0.014914262
41 0.014895615
42 0.014557817
43 0.01448713
44 0.01466586
45 0.014728668
46 0.01481263
47 0.014749491
48 0.014702504
49 0.014654055
50 0.014483963
51 0.014531551
52 0.014243385
53 0.014356601
54 0.014368214
55 0.014484126
56 0.014689535
57 0.014737458
58 0.014937159
59 0.01480438
60 0.01704201
61 0.016122121
62 0.014920484
63 0.015188287
64 0.0151745835
65 0.015440951
66 0.015456532
67 0.0151623
68 0.015033282
69 0.014762313
70 0.014678031
71 0.014655777
72 0.014800668
73 0.014763852
74 0.01485842
75 0.0149348155
76 0.014689899
77 0.0146396905
78 0.014750918
79 0.014614595
80 0.01462612
81 0.014856691
82 0.014988969
83 0.015030388
84 0.014973486
85 0.014862659
86 0.014603311
87 0.0145554375
88 0.014566473
89 0.014537498
90 0.014630836
91 0.014590002
92 0.014697739
93 0.014690195
94 0.014578691
95 0.014945134
96 0.014725394
97 0.014536246
98 0.014584576
99 0.014694228
100 0.014853049


==> Figures/results/fandisk_step_vs_rmse_tonemapped_abs.tex <==
0 0.17002928
1 0.09572428
2 0.029559681
3 0.023923637
4 0.022797795
5 0.018490735
6 0.015562384
7 0.01602713
8 0.014167961
9 0.014642671
10 0.012961994
11 0.010851872
12 0.011161404
13 0.011029002
14 0.010941123
15 0.01059602
16 0.011023184
17 0.010681065
18 0.009999187
19 0.0119691035
20 0.011472841
21 0.011449249
22 0.011458604
23 0.010772525
24 0.010764652
25 0.009879091
26 0.010547827
27 0.011177245
28 0.010830565
29 0.010731147
30 0.010705475
31 0.010398838
32 0.009862822
33 0.009777896
34 0.009944279
35 0.009902041
36 0.010429344
37 0.010442608
38 0.010353378
39 0.00946935
40 0.009513505
41 0.009304288
42 0.0096854
43 0.009631923
44 0.009786247
45 0.011119756
46 0.0105979135
47 0.0106441155
48 0.010871492
49 0.009388443
50 0.0089647155
51 0.009229208
52 0.008937341
53 0.00837072
54 0.008432492
55 0.008644731
56 0.008479795
57 0.008661044
58 0.008736446
59 0.008450835
60 0.008401683
61 0.008573707
62 0.008768465
63 0.009188064
64 0.009398701
65 0.010227437
66 0.010422794
67 0.010064937
68 0.013643568
69 0.011399288
70 0.011603362
71 0.011516687
72 0.011584152
73 0.011317121
74 0.010977275
75 0.01079719
76 0.010425905
77 0.01084459
78 0.010431051
79 0.010087721
80 0.010056439
81 0.009790961
82 0.0100408485
83 0.009455944
84 0.009626146
85 0.009563294
86 0.009206994
87 0.009560729
88 0.011388799
89 0.011203541
90 0.009941531
91 0.009737735
92 0.009932492
93 0.009293468
94 0.009227946
95 0.009262776
96 0.0091827335
97 0.008120901
98 0.008340322
99 0.008242857
100 0.008324375


==> Figures/results/knots_step_vs_rmse_tonemapped_abs.tex <==
0 0.20442861
1 0.05984244
2 0.049179144
3 0.044628114
4 0.036129694
5 0.032619122
6 0.030167123
7 0.029043894
8 0.02769713
9 0.026622444
10 0.025444373
11 0.024981596
12 0.02406262
13 0.023475634
14 0.022852158
15 0.02250065
16 0.02225758
17 0.02136204
18 0.021662321
19 0.021725522
20 0.021522215
21 0.020749094
22 0.02058015
23 0.019954683
24 0.020239979
25 0.02011948
26 0.019941622
27 0.01983271
28 0.019874385
29 0.020087786
30 0.019917464
31 0.019679043
32 0.01971965
33 0.019794555
34 0.019371197
35 0.019650863
36 0.019410556
37 0.019326901
38 0.01921832
39 0.01906727
40 0.019446703
41 0.019717637
42 0.01926307
43 0.01928206
44 0.019071283
45 0.018898567
46 0.01895066
47 0.019430786
48 0.01917385
49 0.019285874
50 0.019170137
51 0.019328738
52 0.01963652
53 0.019538708
54 0.019756729
55 0.019572048
56 0.020119013
57 0.020531757
58 0.019546976
59 0.019449444
60 0.019435132
61 0.019334719
62 0.019405847
63 0.019189341
64 0.01944524
65 0.01970484
66 0.019704994
67 0.019772349
68 0.019640146
69 0.019454233
70 0.019613432
71 0.019556923
72 0.020098172
73 0.019929204
74 0.018908178
75 0.018945372
76 0.01886055
77 0.018767243
78 0.018835919
79 0.018861545
80 0.018964384
81 0.018897321
82 0.0190047
83 0.019218503
84 0.01914059
85 0.019274468
86 0.019048957
87 0.019000875
88 0.019049164
89 0.01895285
90 0.01872612
91 0.019286701
92 0.01931286
93 0.018991396
94 0.018895136
95 0.019101499
96 0.019118574
97 0.018689314
98 0.018929683
99 0.018996058
100 0.020281617


==> Figures/results/sculpture_step_vs_rmse_tonemapped_abs.tex <==
0 0.39074966
1 0.13329217
2 0.07926395
3 0.063578375
4 0.055780426
5 0.05462557
6 0.051295087
7 0.047430865
8 0.044897616
9 0.04353704
10 0.042098217
11 0.0411227
12 0.039445188
13 0.036243252
14 0.034557506
15 0.03330083
16 0.0322519
17 0.03248568
18 0.041502226
19 0.042721193
20 0.03982226
21 0.037454784
22 0.036133327
23 0.035816822
24 0.035369754
25 0.034683317
26 0.034098323
27 0.033463836
28 0.0335939
29 0.033209104
30 0.033064168
31 0.03446269
32 0.033888068
33 0.033749547
34 0.03389374
35 0.03346588
36 0.033127155
37 0.032855764
38 0.03270013
39 0.033404116
40 0.03255178
41 0.032338638
42 0.032258563
43 0.03238742
44 0.03212505
45 0.03227741
46 0.032953184
47 0.033833314
48 0.032902718
49 0.032456003
50 0.03241564
51 0.032282397
52 0.03189868
53 0.03150864
54 0.03120722
55 0.031571504
56 0.03106904
57 0.03187181
58 0.031691078
59 0.032341104
60 0.031542078
61 0.031511072
62 0.031458165
63 0.031709943
64 0.03194542
65 0.032246575
66 0.0313652
67 0.030929461
68 0.030990088
69 0.030936355
70 0.030954694
71 0.03129488
72 0.03128785
73 0.031471208
74 0.031548724
75 0.031522866
76 0.031504676
77 0.03134038
78 0.03208905
79 0.031413916
80 0.03140678
81 0.031554367
82 0.03144072
83 0.031196669
84 0.03127361
85 0.030803379
86 0.031226136
87 0.031183166
88 0.030995056
89 0.03088095
90 0.030950783
91 0.030933028
92 0.030735148
93 0.030770501
94 0.03088818
95 0.030931933
96 0.030561442
97 0.03094329
98 0.031035649
99 0.030954987
100 0.030891923

